A Proximal Quasi-Newton Trust-Region Method for Nonsmooth Regularized Optimization

We develop a trust-region method for minimizing the sum of a smooth term $f$ and a nonsmooth term $h$), both of which can be nonconvex. Each iteration of our method minimizes a possibly nonconvex model of $f + h$ in a trust region. The model coincides with $f + h$ in value and subdifferential at the center. We establish global convergence to a first-order stationary point when $f$ satisfies a smoothness condition that holds, in particular, when it has Lipschitz-continuous gradient, and $h$ is proper and lower semi-continuous. The model of $h$ is required to be proper, lower-semi-continuous and prox-bounded. Under these weak assumptions, we establish a worst-case $O(1/\epsilon^2)$ iteration complexity bound that matches the best known complexity bound of standard trust-region methods for smooth optimization. We detail a special instance, named TR-PG, in which we use a limited-memory quasi-Newton model of $f$ and compute a step with the proximal gradient method, resulting in a practical proximal quasi-Newton method. We establish similar convergence properties and complexity bound for a quadratic regularization variant, named R2, and provide an interpretation as a proximal gradient method with adaptive step size for nonconvex problems. R2 may also be used to compute steps inside the trust-region method, resulting in an implementation named TR-R2. We describe our Julia implementations and report numerical results on inverse problems from sparse optimization and signal processing. Both TR-PG and TR-R2 exhibit promising performance and compare favorably with two linesearch proximal quasi-Newton methods based on convex models.

==> figs/ls/2/ls.tex <==
\begin{tabular}{| c |c |c || c |c |c |c |}
    \hline
Minima    % Table header
    \rowcolor[gray]{0.9}
   & Function & TR & PG & True \\
    \hline
    % Table body
  \rowcolor[gray]{0.7}
     & $ (f + h)(x) $ & 0.000 & 0.540 & 0.000 \\
  \rowcolor[gray]{0.8}
     & $ f(x) $ & 0.000 & 0.540 & 0.000 \\
  \rowcolor[gray]{0.7}
     & $ h(x) $ & 0.000 & 0.000 & 0.000 \\
  \rowcolor[gray]{0.8}
     & $ ||x - x_0||_2 $ & 0.002 & 6.992 & 0.000 \\
\end{tabular}


==> figs/ls/3/ls.tex <==
\begin{tabular}{| c |c |c || c |c |c |c |}
    \hline
Minima    % Table header
    \rowcolor[gray]{0.9}
   & Function & TR & PG & True \\
    \hline
    % Table body
  \rowcolor[gray]{0.7}
     & $ (f + h)(x) $ & 0.000 & 0.681 & 0.000 \\
  \rowcolor[gray]{0.8}
     & $ f(x) $ & 0.000 & 0.681 & 0.000 \\
  \rowcolor[gray]{0.7}
     & $ h(x) $ & 0.000 & 0.000 & 0.000 \\
  \rowcolor[gray]{0.8}
     & $ ||x - x_0||_2 $ & 0.002 & 9.050 & 0.000 \\
\end{tabular}


==> subproblem.tex <==
\section{Solution of the trust-region subproblem}%
\label{sec:subproblem}



